CUDA Agent: Large-Scale Agentic RL for High-Performance CUDA Kernel Generation

GPU kernel optimization is fundamental to modern deep learning but remains a highly specialized task requiring deep hardware expertise. Despite strong performance in general programming, large language models (LLMs) remain uncompetitive with compiler-based systems such as torch.compile for CUDA kernel generation. Existing CUDA code generation approaches either rely on training-free refinement or fine-tune models within fixed multi-turn execution-feedback loops, but both paradigms fail to fundamentally improve the model's intrinsic CUDA optimization ability, resulting in limited performance gains. We present CUDA Agent, a large-scale agentic reinforcement learning system that develops CUDA kernel expertise through three components: a scalable data synthesis pipeline, a skill-augmented CUDA development environment with automated verification and profiling to provide reliable reward signals, and reinforcement learning algorithmic techniques enabling stable training. CUDA Agent achieves state-of-the-art results on KernelBench, delivering 100\%, 100\%, and 92\% faster rate over torch.compile on KernelBench Level-1, Level-2, and Level-3 splits, outperforming the strongest proprietary models such as Claude Opus 4.5 and Gemini 3 Pro by about 40\% on the hardest Level-3 setting.

==> appendices/3_base_model_performance.tex <==
\section{Performance of the Base Model}
\label{appd:base_model_performance}

\subsection{Benchmark Descriptions}
To provide a comprehensive evaluation of our Base Model, we selected a diverse set of benchmarks covering General Knowledge, Reasoning, Math, and Coding. The details of these benchmarks are as follows:

\begin{description}
    \item[MMLU] A comprehensive test covering 57 subjects across STEM, the humanities, the social sciences, and more. It measures the model's general knowledge and problem-solving ability.
    \item[MMLU-Pro] An enhanced and more challenging version of MMLU designed to better discriminate between high-performing models, requiring more robust reasoning capabilities.
    \item[SuperGPQA] An advanced evaluation set focused on graduate-level scientific reasoning, testing the model's ability to answer complex questions in biology, physics, and chemistry.
    \item[BBH] A subset of the BIG-bench task suite, focusing on tasks where language models have historically struggled. It evaluates multi-step reasoning, logical deduction, and algorithmic thinking.
    \item[GPQA-Diamond] A highly difficult benchmark consisting of graduate-level Google-proof Q\&A questions. The "Diamond" subset represents the highest quality and hardest questions, intended to test expert-level scientific knowledge.
    \item[GSM8k] A dataset of high quality linguistically diverse grade school math word problems. It is the standard benchmark for multi-step mathematical reasoning.
    \item[MATH] A dataset of challenging mathematics problems from high school math competitions. It is significantly harder than GSM8k and requires complex problem-solving skills.
    \item[MBPP] A benchmark for evaluating code generation, consisting of crowd-sourced Python programming problems that cover programming fundamentals and standard library usage.
\end{description}

% \subsection{Performance Comparison}
% Table \ref{tab:base_model_benchmarks_v2} presents the performance of our base model compared to LLaMA-4-Maverick Base, DeepSeek-V3 Base, Qwen3-235B-A22B Base, and Kimi-K2 Base. Our base model achieves performance comparable to state-of-the-art open-source models across a diverse set of benchmarks, encompassing general knowledge, logical reasoning, STEM, mathematics, and code generation.

\begin{table}[h!]
\centering
\caption{Comparison of our Base Model with other leading base models. The best results are highlighted in \textbf{bold}. An em dash (—) indicates that the result is not reported. Kimi-K2 Base is reported to achieve 80.33 on EvalPlus (averaging HumanEval, MBPP, HumanEval+, and MBPP+).}
\label{tab:base_model_benchmarks_v2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccc}
\toprule
\textbf{Category} & \textbf{Benchmark} & \textbf{Base Model (Ours)} & \textbf{LLaMA-4-Maverick Base} & \textbf{DeepSeek-V3 Base} & \textbf{Qwen3-235B-A22B Base} & \textbf{Kimi-K2 Base} \\
\midrule
\multirow{4}{*}{\makecell[l]{General Knowledge \\ \& Reasoning}} 
 & MMLU & \textbf{88.83} & 85.16 & 87.19 & 87.81 & 87.79 \\
 & MMLU-Pro & \textbf{69.98} & 63.91 & 59.84 & 68.18 & 69.17 \\
 & SuperGPQA & \textbf{45.08} & 40.85 & 41.53 & 44.06 & 44.67 \\
 & BBH & \textbf{92.08} & 83.62 & 86.22 & 88.87 & 88.71 \\
\midrule
\multirow{4}{*}{\makecell[l]{STEM \& Math \\ \& Coding}} 
 & GPQA-Diamond & 43.43 & 43.94 & 41.92 & 47.47 & \textbf{48.11} \\
 & GSM8k & 93.10 & 87.72 & 87.57 & \textbf{94.39} & 92.12 \\
 & MATH & \textbf{72.86} & 63.32 & 62.62 & 71.84 & 70.22 \\
 & MBPP & \textbf{83.60} & 75.40 & 74.20 & 81.40 & – \\
\bottomrule
\end{tabular}%
}
\end{table}



==> sections/ours_settings.tex <==
%%%%%%%%%%%%%%%%%% Ours %%%%%%%%%%%%%%%%%%
\usepackage{dblfloatfix}
\usepackage{minted}

% \usepackage{markdown}

\newmintinline{python}{python3}
\newminted{python}{frame=single,framesep=1mm,fontsize=\scriptsize,python3,linenos}
\usemintedstyle{colorful}
% 行内 markdown
\newmintinline{md}{markdown}

% markdown 代码块环境
\newminted{mdcode}{
    style=colorful,
    frame=single,
    framesep=1mm,
    fontsize=\scriptsize,
    linenos,
    breaklines,
    tabsize=2
}

\newcommand{\hanlin}[1]{\textcolor{blue}{[Hanlin: #1 ]}}
\newcommand{\weinan}[1]{\textcolor{orange}{[Weinan: #1 ]}}

\newcommand{\ours}{CUDA Agent\xspace}
